"Who can help me?": Knowledge Infused Matching of Support Seekers and Support Providers during COVID-19 on Reddit

During the ongoing COVID-19 crisis, subreddits on Reddit, such as r/Coronavirus saw a rapid growth in user's requests for help (support seekers - SSs) including individuals with varying professions and experiences with diverse perspectives on care (support providers - SPs). Currently, knowledgeable human moderators match an SS with a user with relevant experience, i.e, an SP on these subreddits. This unscalable process defers timely care. We present a medical knowledge-infused approach to efficient matching of SS and SPs validated by experts for the users affected by anxiety and depression, in the context of with COVID-19. After matching, each SP to an SS labeled as either supportive, informative, or similar (sharing experiences) using the principles of natural language inference. Evaluation by 21 domain experts indicates the efficacy of incorporated knowledge and shows the efficacy the matching system.

==> discussion.tex <==
During COVID-19, r/Coronavirus and r/covid19\_support communities have seen an immense increase in traffic. As such, moderators who effectively control the responses and comments on these communities found themselves overwhelmed. Although Reddit is where the issue became evident in our study, individuals suffering from depression or anxiety vent their mental health woes on other social media platforms due to anonymity and free disclosure \cite{yazdavar2020multimodal, saud2020usage}. Some individuals take SPs' role by providing advice, sharing necessary experiences, or information to help SS. Specifically in mental health communities, there are relatively few moderators and the task of associating SSs with SPs is mind-numbing. Thus, the need for a computational approach to address this issue, especially during a crisis, is exigent. 

Consequently, it is crucial to evaluate the SSs and SPs matched by our method from a clinician’s perspective for widespread use across other community-based platforms (e.g. Talklife \cite{kushner2020bursts}). Our research sheds light on building a system to associate SS with SPs to create a peer-support group on community-based platforms \cite{chuang2010social}. Through quantitative and qualitative research, we believe such an approach could cater to early intervention strategy through supportive and information content that SS receives from individuals of diverse backgrounds. Future work focuses on exploring other pairs of subreddits: (r/Opiates, r/OpiatesRecovery), (r/CripplingAlcoholism, r/StopDrinking), and (r/SelfHarm, r/StopSelfHarm). Also, we posit the need for changes in qualitative practical clinician evaluation.  This includes asking the following questions: (a) Of the numbers you think as relevant, would you be able to pick at least one user with whom you feel the support seeker can have a meaningful conversation? (b) Do you think the support seeker will have gained trust in the support provider based on the contextual overlap between the described problem and the solution provided? \cite{han2018hybrid} (c) Do you think the support provider's response would have a negative impact on the user seeking support? The answers to the above questions would bolster the ability of our method to match the right SSs with SPs such that the issue is resolved in terms of (1) expressing overcoming a similar problem by the SP, (2) providing a perspective by the SP that is helpful as a plausible alternative to the SS or (3) providing information that is in general use to the SS’s issue.

==> simulation_results.tex <==

%\begin{figure*}[!ht]
%    \centering
%    \vspace{-1em}
%    \includegraphics[width=\textwidth]{simulation_model.png}
%    \caption{Simulation Setting}
%    \label{fig:simulation}
%\end{figure*}
%AS: "We know also that there are 108SP users." We should mention how we came up with these, these are results of thresholding(Pr(0.7)) or we used these from suicide risk dataset.
\subsection{Relevance to Reddit data} We see in Table \ref{tab:data-stats}, that there $9.5$K SS users labeled using the classifier. We know also that there are $108$ SP users. To set the simulation settings to be reflective of real world Reddit data, we also perform a sanity check by measuring the overlap in the medical concepts between SS and SP posts related to COVID-19 subreddits to see if there is content overlap. Without content overlap it would not make sense to match them. Let $C_{SS}^{l}$ and $C_{SP}^{l}$ be the concepts in the lexicon $l,~l \in \{l1,l2\}$ pertaining to the SS and SP posts respectively. An example of the lexicons and the concepts can be seen in Table \ref{tab:lexicon}. We compute overlap between the concepts as: \[\mathcal{O} = \frac{|C_{SS}^{l1} \cap C_{SP}^{l1}|}{|C_{SS}^{l1} \cup C_{SP}^{l1}|} + \frac{|C_{SS}^{l2} \cap C_{SP}^{l2}|}{|C_{SS}^{l2} \cup C_{SP}^{l2}|}\] Figure \ref{fig:figure tsne_overlap} shows a TSNE visualization of the concepts for the SSs and SPs for all the users in the subreddits. We observe that there is significant ($>60\%$) overlap as computed by $\mathcal{O}*100$ for the $9.5$K SSs and $108$ SPs that are part of our filtered dataset. We also observe that a potential SS match with an SP takes $\leq 20$ interactions. 

\begin{table}[!htbp]
\begin{tabular}{p{1.5cm}|p{6.5cm}}
\toprule[1.5pt]
\textbf{Lexicon} & \textbf{ Concepts} \\\midrule[1pt]
Anxiety & petrified, shaken, terrified, fear, scared, panicky, on edge, with my stomach in knots, fretful, tense, edgy, antsy, Troubled, panic attacks, hopelessness, physical sensations,
social phobia, fear of eating in public,fear of public washing, school phobia, agoraphobia, etc. \\
Depression & absence of pleasure, anhedonia, apathy, boredom, dissatisfaction, hatred, depressed mood, dejection, melancholy, feeling blah, nothing to live for, feeling blue, low spirits, depressive symptoms, depressed mood, loss of interest, dysthymia, major Depression, affective disorder, psychotic depression, etc. \\
\bottomrule[1.5pt]
\end{tabular}
\caption{Example concepts in the Anxiety ($l1$) and Depression ($l2$) lexicon used to study the posts from SSs and SPs.}
\label{tab:lexicon}
\vspace{-1em}
\end{table}

\subsection{Simulation Settings}Let $N,~M$ and $K$ be the number of SSs, SPs, and max number of matches that a SS has with an SP from the initial point of contact. We set $N = 10000$, $M=108$, and $K=20$ to reflect the true numbers on the Reddit platform. %We perform simulation with the architecture as shown in figure \ref{fig:simulation}. 
We set conditions $C1, .. Cp$ randomly from $\{0,1\}$ to simulate affliction of SS from an illness such as anxiety and depression. Similarly, we set recoveries $R1,...Rp \sim Uniform(0,1)$, to simulate that SPs have recovered from the afflictions to varying degrees (skills and experiences). A good match is simulated by a rating calculated using \[\mathcal{R} = \frac{\sum_{p}Cp\cdot Rp}{\sum_{p}Cp}\]The different selection strategies choose an SP for an SS to match. Random selection chooses at random (R), Probabilistic Greedy (PG) selection chooses the best rated, and KI selection chooses the best rated as computed using knowledge. We use three context-specific metrics, developed with the help of DEs, to measure the simulation's performance. 
\begin{itemize}
    \item Rating's Stability:  The average log variance of $\mathcal{R}$ in the last 20 matches. 
    \item \#IdleSPs: Number of support providers who are idle at any given point in time before SS initiates an interaction. 
    \item TGM: Number of matches between SS and SPs before an SS identifies a relevant SP. 
\end{itemize}
We see in table \ref{tab:1} that \emph{KI} shows convincing improvements in the simulation. With this evidence, we proceed to testing KI match prediction between SSs and SPs on real world Reddit data.

\begin{table}[t]
    \centering
    \begin{tabular}{p{2.2cm}p{2.5cm}p{1cm}p{1.2cm}}
        \toprule[1.2pt]
         Method & Rating's Stability & \#IdleSPs & TGM\\ \midrule
         R & -41.09 & 99.5\%& $>20$ \\
         PG & -26.03 &99.5\% & $>20$ \\
         KI Feature & -9.00 & 18.5\% & 2/20 \\ 
         \bottomrule[1pt]
    \end{tabular}
    \caption{For rating stability we measure log(variance). Since maximum variance in ratings 1.0, optimal rating stability is 0.0 (higher the better). For \#IdleSPs represents the percentage of Idle SPs while matching in process (lower the better). Time to Good Match (TGM) measures how long it took for ratings to stabilize (lower the better). All the measures are averaged across SSs and SPs.}
    %Measuring rating stability, Idle \textcolor{red}{make it relative} (low is good) (mention, minimum and maximum) \textcolor{red}{average time delay} \textcolor{red}{define MRO in experiments} }
    \label{tab:1}
    \vspace{-2em}
\end{table}

